Distilling Knowledge from Reader to Retriever for Question Answering

The task of information retrieval is an important component of many natural language processing systems, such as open domain question answering. While traditional methods were based on hand-crafted features, continuous representations based on neural networks recently obtained competitive results. A challenge of using such methods is to obtain supervised data to train the retriever model, corresponding to pairs of query and support documents. In this paper, we propose a technique to learn retriever models for downstream tasks, inspired by knowledge distillation, and which does not require annotated pairs of query and documents. Our approach leverages attention scores of a reader model, used to solve the task based on retrieved documents, to obtain synthetic labels for the retriever. We evaluate our method on question answering, obtaining state-of-the-art results.

==> macros.tex <==

\newcommand{\wt}[1]{\widetilde{ #1 } }
\newcommand{\wh}[1]{\widehat{ #1 } }
\newcommand{\A}{\mathcal{A}}
\newcommand{\TV}{\mathrm{TV}}
\newcommand{\LB}{\mathrm{LB}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\CCC}{\mathcal{C}}
% \newcommand{\R}{\mathbb{R}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\DBB}{\mathcal{B}^{\brac{1}}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\bxi}{\bar{\xi}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\Ind}{\mathbf{1}}
\newcommand{\Noi}{\cN}
\newcommand{\perm}{\mathfrak{S}}

% Carlos
\newcommand{\cfg}[1]{\textcolor{blue}{#1}}
\newcommand{\bdb}[1]{\textcolor{red}{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\MAT}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\VEC}[1]{\left[\begin{array}{c} #1 \end{array}\right]}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\keys}[1]{\left\{ #1 \right\}}
\newcommand{\sqbr}[1]{\left[ #1 \right]}
\newcommand{\brac}[1]{\left( #1 \right) }
\newcommand{\ml}[1]{\mathcal{ #1 } }
\newcommand{\op}[1]{ \operatorname{#1} }
\newcommand{\normInf}[1]{\left\| #1 \right\| _{\infty}}
\newcommand{\normTwo}[1]{\left\| #1 \right\| _{2}}
\newcommand{\normOne}[1]{\left\| #1 \right\| _{1}}
\newcommand{\normTV}[1]{\left\| #1 \right\| _{\op{TV}}}
\newcommand{\normF}[1]{\left\| #1 \right\| _{F}}
\newcommand{\atomicnorm}[1]{\left\| #1 \right| \right|_{\mathcal{A}}}
\newcommand{\der}[2]{\frac{\text{d}#2}{\text{d}#1}}
\newcommand{\derTwo}[2]{\frac{\mathrm{d} ^2#2}{\mathrm{d}#1^2}}
\newcommand{\set}[2]{ \keys{ #1 \; | \; #2 } }
\newcommand{\PROD}[2]{\left \langle #1, #2\right \rangle}
\newcommand{\diff}[1]{ \, \text{d} #1 }
\newcommand{\real}{\op{Re}}
\newcommand{\imag}{\op{Im}}
\newcommand{\sgn}{\text{sgn}}





==> tables.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lccccc}
  \toprule
  Method & P@5 & P@20 & P@100 & Dev EM & Test EM \\
         
  \midrule
  DPR~\citep{karpukhin2020dense} & 67.1** & 79.4 & 86.0 & 46.5 & 48.2 \\
  ColBERT-QA$_{0}$~\citep{khattab2020relevanceguided} & 66.2 & - & - \\
  ColBERT-QA$_1$ & 74.9 & - & - \\
  ColBERT-QA$_2$ & 77.4 & - & - \\
  \midrule
  MSE Regression First iteration & ~61 & - & - \\
  MSE Regression Second iteration & 71.3 & - & 87.6\\
  MSE Regression Third iteration & 66.0 & - & -\\
  Ranking Loss First Iteration & 67.5 & 80.0 & 86.8  \\
  Ranking Loss Second Iteration & 68.2 & 80.7 & 86.9  \\
  Ranking Loss Second Iteration w reader finetuning & 71.9 & 82.7 & 88.5 & 48.2 & 49.3 \\
  Ranking Loss Third Iteration w reader finetuning & 72.6 & 83.0 & 88.4 & 48.2 & 49.3 \\
  KL Divergence First Iteration & 69.1 & 81.4 & 87.8 & 47.8 & 49.6 \\
  KL Divergence Second Iteration & 72.8 & 83.4 & 89.1 & 48.2 & 50.1 \\
  KL Divergence First Iteration 5x154 & 70.4 & 81.8 & 88.2 & \\
  KL Divergence First Iteration 5x768 & 70.5 & 81.9 & 88.4 & \\
  \midrule
  KL Divergence First Iteration dropout 0.01 & 70.0 & 81.8 & 88.2 \\
  KL Divergence First Iteration dropout 0.05 & 69.5 & 81.7 & 88.0 \\
  \midrule
  KL Divergence First Iteration 40 passages & 68.3 & 80.2 & 87.2 \\
  Marge 40 passages starting from KL Iter1 retriever & 52.5 & 65.6 & 76.0 \\
  \bottomrule
\end{tabular}
\caption[Caption]{Retrieval performance measured as the proportion of questions for which at least one of the top-k retrieved passage contains the answer.}
\label{tab:sota}
\end{table*}


\begin{table*}[t]
\centering
\begin{tabular}{lccccc}
  \toprule
  Method & P@5 & P@20 & P@100 & Dev EM & Test EM \\
         
  \midrule
  DPR~\citep{karpukhin2020dense} & - & 79.4 & 85.0 & 64.6 & 65.0 \\
  ColBERT-QA$_{0}$~\citep{khattab2020relevanceguided} & 72.4 & - & - \\
  ColBERT-QA$_1$ & 80.1 & - & - \\
  ColBERT-QA$_2$ & 81.1 & - & - \\
  \midrule
  KL Divergence First Iteration & 74.0 & 81.3 & 86.2 & 67.1 & 68.2 \\
  PQ 64 subquantizers 8 bits & 71.4 & 79.3 & 85.0 \\
  PQ 128 subquantizers 8 bits & 72.2 & 80.3 & 85.6 \\
  \midrule
  KL Divergence Second Iteration & 76.3 & 83.5 & 87.3 & 68.1 & 69.0 \\
  
\end{tabular}
\caption[Caption]{TriviaQA.}
\label{tab:sota}
\end{table*}


\begin{table*}[t]
\centering
\begin{tabular}{lccccc}
  \toprule
   & FiD base & DPR doc. & BM25 doc. & Bert doc. \\
  \midrule
  NQ & 48.2 & 50.1 & 48.9 & 40.8 \\ 
  TriviaQA & 65.0 & 69.0 & (67.0?) & -\\
\end{tabular}
\caption[Caption]{TriviaQA.}
\label{tab:sota}
\end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{lccccc}
  \toprule
  Method & Rouge-L & Bleu-1 & Bleu-4 & Meteor\\
  \midrule
  Best result original paper & 14.5 & 20.0 & 2.23 & 4.6 \\
  \midrule
  10 passages & 26.9 & 30.2 & 5.4 & 9.0 \\
  20 passages & 28.3 & 31.0 & 6.0 & 9.4 \\
  train 20 test 50 & 29.6 & 31.7 & 6.2 & 9.7 \\
  50 passages & 29.0 & 29.1 & 5.7 & 9.5 \\
  \midrule
  20 passages trained retriever & 30.4 & 32.3 & 5.9 & 10.0
\end{tabular}
\caption[Caption]{Performance on NarrativeQA evaluation set.}
\label{tab:sota}
\end{table*}

